FMM-Net: neural network architecture based on the Fast Multipole Method

In this paper, we propose a new neural network architecture based on the H2 matrix. Even though networks with H2-inspired architecture already exist, and our approach is designed to reduce memory costs and improve performance by taking into account the sparsity template of the H2 matrix. In numerical comparison with alternative neural networks, including the known H2-based ones, our architecture showed itself as beneficial in terms of performance, memory, and scalability.

==> FMM-Net (Version 200)/figs/L_lvl_compr.tex <==
\resizebox{\textwidth}{!}{
\tikz{
    \foreach \i in {0,...,15}
    {
        \foreach \j in {0,...,4}
        {
            \pgfmathtruncatemacro{\r}{int(\closeDots[\i][\j])}
            \pgfmathtruncatemacro{\ii}{int(\closeDots[\i][0])}
            \draw [blue!50!white,fill=blue!50!white,opacity=1.0](\r,15-\ii) rectangle ++(1,1);
            % \node [scale=4][draw] at (\r,16-0) {\Huge{R: \r}};
        }
    }
    \draw[step=1cm,gray!20!white] (0,0) grid (16,16);
    \draw[gray!80!white] (0,0) rectangle (16,16);
    \node [scale=4] at (8,-2) { $C$};


    \begin{scope}[shift={(20,0)}]

            \foreach \i in {0,...,16}
            {
                \draw[gray!20!white] (0,\i)--(8,\i);
                \draw[gray!20!white] (\i*0.5,0) -- (\i*0.5,16);
            }
            \foreach \i in {0,...,15}
            {
            \draw[green!50!white,fill=green!50!white](\i*0.5,15-\i) rectangle ++(0.5,1);
            }
            \node [scale=4] at (4,-2) {$U_L$ };
            \draw[gray!80!white] (0,0) rectangle (8,16);
    \end{scope}
    \begin{scope}[shift={(30,0)}]
            \fill[blue!20!white]  (0,8) rectangle (8,16);
            \foreach \i in {0,...,15}
            {
                \foreach \j in {0,...,4}
                {
                    \pgfmathtruncatemacro{\r}{int(\closeDots[\i][\j])}
                    \pgfmathtruncatemacro{\ii}{int(\closeDots[\i][0])}
                    \draw [white,fill=white,opacity=1.0](\r*0.5,15.5-\ii*0.5) rectangle ++(0.5,0.5);
                    % \node [scale=4][draw] at (\r,16-0) {\Huge{R: \r}};
                }
            }
            \draw[step=1cm,gray!20!white] (0,8) grid (8,16);
            \draw[gray!80!white] (0,8) rectangle (8,16);
            \node [scale=4] at (4,6) {  $\widehat{M}_L$ };
    \end{scope}
    \begin{scope}[shift={(40,0)}]
        \foreach \i in {0,...,16}
        {
            \draw[gray!20!white] (0,\i*0.5+8)--(16,\i*0.5+8);
            \draw[gray!20!white] (\i,8) -- (\i,16);
        }
        \foreach \i in {0,...,15}
        {
        \draw[green!50!white,fill=green!50!white](\i,15.5-\i*0.5) rectangle ++(1,0.5);
        }
        \node [scale=4] at (8,6) {  $V_L$ };
        \draw[gray!80!white] (0,8) rectangle (16,16);
    \end{scope}
    \node [scale=4] at (18,8) {  + };
    \node [scale=4] at (29,12) {  * };
    \node [scale=4] at (39,12) {  * };
}
}


==> FMM-Net (Version 200)/figs/bottom_level_compression.tex <==
\tikz{
  % \begin{scope}[shift={(-8,0)}]
     \fill[blue!20!white]  (0,0) rectangle (16,16);
     % \fill[blue!50!white] (4,4) rectangle (5,5) ;
    \foreach \i in {0,...,15}
    {
        \foreach \j in {0,...,4}
        {
            \pgfmathtruncatemacro{\r}{int(\closeDots[\i][\j])}
            \pgfmathtruncatemacro{\ii}{int(\closeDots[\i][0])}
            \draw [white,fill=white,opacity=1.0](\r,15-\ii) rectangle ++(1,1);
        }
    }

    \draw[white,fill=white] (0,15) rectangle (16,15.5);
    \draw[white,fill=white] (3.5,0) rectangle (4,16);
    \draw[step=1cm,gray!20!white] (0,0) grid (16,16);

    \draw[green!50!white,fill=green!50!white](-2.5, 15) rectangle ++(0.5,1);
    \draw[green!50!white,fill=green!50!white](3,17) rectangle ++(1,0.5);

    \node [scale=2, above] at (3.5,17.5) {$\widetilde{V}_j$};
    \node [scale=2, left] at (-2.5,15.5) {$\widetilde{U}_i$};
    \node [scale=2] at (1.5,16.5) {$\widetilde{F}_{ij}$};
    \draw[-latex,line width=1mm ] (2,16.5) -- (3.25,15.75);
    % \draw[-latex,line width=1mm ] (-2,14.5) -- (0.5,14.5);
    % \node [scale=3,left] at (-2,11.5) {Far block};
    % \draw[-latex,line width=1mm ] (-2,11.5) -- (0.5,11.5);
    % \draw[white] (24,0) rectangle ++(1,1);
}


==> FMM-Net (Version 200)/figs/ce_table.tex <==
 \begin{tabular}{||c c c c c||}
 \hline
 $N$ & h2nn &  MNN-$\mathcal{H}^2$-Mix &  MNN-$\mathcal{H}^2$-LC& conv\\
 \hline\hline
 320 &  0.00790/0.00789 &   0.00857/0.00858 &   0.00218/0.00218&0.26599/0.26600\\
 640 &  0.00424/0.00425 &  0.14413/0.14592 &   0.10721/0.11022&0.27551/0.27860\\
 1280 &   0.01464/0.00425 &  0.19069/0.19070 &   0.22265/0.22287&0.33206/0.33301 \\ [1ex]
 \hline
\end{tabular}


==> FMM-Net (Version 200)/figs/ce_table_time.tex <==
 \begin{tabular}{||c c c c c||}
 \hline
 $N$ & h2nn &  MNN-$\mathcal{H}^2$-Mix &  MNN-$\mathcal{H}^2$-LC & conv\\
 \hline\hline
 320 &    3.9095 &   2.5115 &   0.7676 & 1.0347\\
 640 &    8.6155 &   4.4554 &   1.3959 & 2.2322\\
 1280 &   18.653 &   9.9784 &   2.5016 & 4.2035\\ [1ex]
 \hline
\end{tabular}



==> FMM-Net (Version 200)/figs/close_mat.tex <==
\def\closeDots{{{ 0, 10,  5,  2,  1},
        {1, 11,  0,  3,  4},
        {4, 14,  1,  6,  5},
        {5, 15,  4,  7,  0},
        {2,  0,  7,  8,  3},
        {3,  1,  2,  9,  6},
        {6,  4,  3, 12,  7},
        {7,  5,  6, 13,  2},
        {8,  2, 13, 10,  9},
        {9,  3,  8, 11, 12},
       {12,  6,  9, 14, 13},
       {13,  7, 12, 15,  8},
       {10,  8, 15,  0, 11},
       {11,  9, 10,  1, 14},
       {14, 12, 11,  4, 15},
       {15, 13, 14,  5, 10}}}

\def\RandDots{{{0.48637352, 0.53586711, 0.87386436, 0.92523105, 0.19662421,
               0.11208547, 0.34445174, 0.14922475, 0.19785328, 0.63301906,
               0.25910754, 0.58501838, 0.88157351, 0.05393866, 0.31015342,
               0.08242764, 0.72402543, 0.61453043, 0.7415675 , 0.86744318},
              {0.94352635, 0.55941481, 0.66484183, 0.82699268, 0.16481487,
               0.52753435, 0.34134099, 0.56140683, 0.67282776, 0.93078796,
               0.30185688, 0.77235954, 0.7517697 , 0.93256297, 0.48900417,
               0.43782538, 0.12732212, 0.90118619, 0.56294379, 0.93998838}}}
\def\RandDotsT{{{0.8245779 , 0.76174813, 0.80744847, 0.97529873, 0.22327913,
               0.62019291, 0.15440187, 0.01456596, 0.82576358, 0.49669774,
               0.13688487, 0.55712594, 0.36549842, 0.84218367, 0.26413289,
               0.37919453, 0.72994362, 0.36359501, 0.63787649, 0.15465958},
              {0.56214302, 0.16206764, 0.26705701, 0.88304504, 0.566555  ,
               0.14174434, 0.61395399, 0.22522736, 0.56733802, 0.07072593,
               0.53008812, 0.93976755, 0.55426911, 0.05349953, 0.02133711,
               0.74527227, 0.94190781, 0.12909986, 0.84066342, 0.39037355}}}


==> FMM-Net (Version 200)/figs/f_l1.tex <==
\begin{figure}[H]
\centering
    \resizebox{0.4\textwidth}{!}{
    \tikz{
        \fill[white]  (0,0) rectangle (16,16);
        \foreach \i in {0,...,3}{
            \fill[blue!20!white]  (\i*4,\i*4) rectangle ++(4cm,4cm);
        }
        \foreach \i in {0,...,15}
        {
            \foreach \j in {0,...,4}
            {
                \pgfmathtruncatemacro{\r}{int(\closeDots[\i][\j])}
                \pgfmathtruncatemacro{\ii}{int(\closeDots[\i][0])}
                \draw [white,fill=white,opacity=1.0](\r,15-\ii) rectangle ++(1,1);
            }
        }
        \draw[step=1cm,gray!20!white] (0,0) grid (16,16);
        \draw[gray!80!white] (0,0) rectangle (16,16);
        \draw[step=4cm,gray,line width=0.34mm ] (0,0) grid (16,16);
        % \node [scale=3,left] at (-2,3.5) {Far block};
        % \draw[-latex,line width=1mm ] (-2,3.5) -- (0.5,3.5);
        % \node [scale=3,left] at (-2,11.5) {Interaction list};
        % \draw[-latex,line width=1mm ] (-2,11.5) -- (0.5,11.5);
        % \draw[white] (24,0) rectangle ++(1,1);
    }
    }
    \caption{Matrix $F_{L-1}$}
    \label{fig:inter_list}
\end{figure}


==> FMM-Net (Version 200)/figs/inter_list.tex <==
    \tikz{
        \fill[blue!50!green, opacity=0.3]  (0,0) rectangle (16,16);
        \foreach \i in {0,...,3}{
            \fill[blue!20!white]  (\i*4,\i*4) rectangle ++(4cm,4cm);
        }
        \foreach \i in {0,...,15}
        {
            \foreach \j in {0,...,4}
            {
                \pgfmathtruncatemacro{\r}{int(\closeDots[\i][\j])}
                \pgfmathtruncatemacro{\ii}{int(\closeDots[\i][0])}
                \draw [white,fill=white,opacity=1.0](\r,15-\ii) rectangle ++(1,1);
            }
        }
        \draw[step=1cm,gray!20!white] (0,0) grid (16,16);
        \draw[gray!80!white] (0,0) rectangle (16,16);
        \draw[step=4cm,gray,line width=0.34mm ] (0,0) grid (16,16);
        \node [scale=3,left] at (-2,2) {Block of $F_{L-1}$};
        \draw[-latex,line width=1mm ] (-2,2) -- (2,2);
        \node [scale=3,left] at (-2,10) {Block of interaction list $M_L$};
        \draw[-latex,line width=1mm ] (-2,10) -- (2,10);
        \draw[white] (30,0) rectangle ++(1,1);
    }


==> FMM-Net (Version 200)/figs/mat_A.tex <==
\tikz{
     \fill[blue!20!white]  (0,0) rectangle (16,16);
    \foreach \i in {0,...,15}
    {
        \foreach \j in {0,...,4}
        {
            \pgfmathtruncatemacro{\r}{int(\closeDots[\i][\j])}
            \pgfmathtruncatemacro{\ii}{int(\closeDots[\i][0])}
            \draw [blue!50!white,fill=blue!50!white,opacity=1.0](\r,15-\ii) rectangle ++(1,1);
        }
    }
    \draw[step=1cm,gray!20!white] (0,0) grid (16,16);
    \node [scale=3,left] at (-2,14.5) {Block of close matrix $C$};
    \draw[-latex,line width=1mm ] (-2,14.5) -- (0.5,14.5);
    \node [scale=3,left] at (-2,11.5) {Block of far matrix $F_L$};
    \draw[-latex,line width=1mm ] (-2,11.5) -- (0.5,11.5);
    \draw[white] (30,0) rectangle ++(1,1);
}


==> FMM-Net (Version 200)/figs/matvec.tex <==
\pgfmathsetmacro{\r}{0.7}
\pgfmathsetmacro{\scale}{2.5}
\pgfmathsetmacro{\ps}{10}
    \tikz{
        \draw[gray] (0*\ps,0*\ps) circle (\r cm);
        \node [scale=\scale] at (0*\ps,0*\ps) {$q$};
        \draw[draw=gray] (1*\ps,0*\ps) circle (\r cm);
        \node [scale=\scale] at (1*\ps,0*\ps) {$w$};
        \draw[-latex,line width=0.5mm ,draw=gray] (0.2*\ps ,0*\ps) -- (0.8*\ps,0*\ps);
        \node [scale=\scale, above] at (0.5*\ps,0*\ps) {$C$};
        \draw[-latex,line width=0.5mm, draw=gray] (0*\ps,0.08*\ps) -- (0*\ps,0.26*\ps);
        \node [scale=\scale, left] at (0*\ps,0.18*\ps) {$V_L$};
        \draw[latex-,line width=0.5mm, draw=gray] (1*\ps,0.08*\ps) -- (1*\ps,0.26*\ps);
        \node [scale=\scale, right] at (1*\ps,0.18*\ps) {$U_L$};

        \begin{scope}[shift={(0,3.4)}]
            \draw[gray] (0*\ps,0*\ps) circle (\r cm);
            \node [scale=\scale] at (0*\ps,0*\ps) {$\hat{q}_L$};
            \draw[draw=gray] (1*\ps,0*\ps) circle (\r cm);
            \node [scale=\scale] at (1*\ps,0*\ps) {$\hat{w}_L$};
            \draw[-latex,line width=0.5mm, draw=gray] (0.2 *\ps,0*\ps) -- (0.8*\ps,0*\ps);
            \node [scale=\scale, above] at (0.5*\ps,0*\ps) {$M_L$};
            \draw[-latex,line width=0.5mm, draw=gray] (0*\ps,0.08*\ps) -- (0*\ps,0.26*\ps);
            \node [scale=\scale, left] at (0*\ps,0.18*\ps) {$V_{L-1}$};
            \draw[latex-,line width=0.5mm, draw=gray] (1*\ps,0.08*\ps) -- (1*\ps,0.26*\ps);
            \node [scale=\scale, right] at (1*\ps,0.18*\ps) {$U_{L-1}$};
        \end{scope}
        \begin{scope}[shift={(0,6.6)}]
            \draw[-latex,line width=0.5mm, draw=gray] (0*\ps,0.08*\ps) -- (0*\ps,0.26*\ps);
            \node [scale=\scale, left] at (0*\ps,0.18*\ps) {$V_{1}$};
            \draw[latex-,line width=0.5mm, draw=gray] (1*\ps,0.08*\ps) -- (1*\ps,0.26*\ps);
            \node [scale=\scale, right] at (1*\ps,0.18*\ps) {$U_{1}$};
        \end{scope}
        \begin{scope}[shift={(0,1*\ps)}]
            \draw[gray] (0*\ps,0*\ps) circle (\r cm);
            \node [scale=\scale] at (0*\ps,0*\ps) {$\hat{q}_1$};
            \draw[draw=gray] (1*\ps,0*\ps) circle (\r cm);
            \node [scale=\scale] at (1*\ps,0*\ps) {$\hat{w}_1$};
            \draw[-latex,line width=0.5mm,draw=gray ] (0.2*\ps ,0*\ps) -- (0.8*\ps,0*\ps);
            \node [scale=\scale, above] at (0.5*\ps,0*\ps) {$M_1$};
        \end{scope}

        \node [scale=\scale] at (0.5*\ps,0.7*\ps) {\dots};
        \node [scale=\scale] at (0*\ps,0.7*\ps) {\vdots};
        \node [scale=\scale] at (1*\ps,0.7*\ps) {\vdots};
    }


==> FMM-Net (Version 200)/figs/nn.tex <==
\pgfmathsetmacro{\r}{0.7}
\pgfmathsetmacro{\scale}{2.5}
\pgfmathsetmacro{\ps}{10}
    \tikz{
        \draw[gray] (0*\ps,0*\ps) circle (\r cm);
        \node [scale=\scale] at (0*\ps,0*\ps) {$q$};
        \draw[draw=gray] (1*\ps,0*\ps) circle (\r cm);
        \node [scale=\scale] at (1*\ps,0*\ps) {$w$};
        \draw[-latex,line width=0.5mm ,draw=gray] (0.2*\ps ,0*\ps) -- (0.8*\ps,0*\ps);
        \node [scale=\scale, above] at (0.5*\ps,0*\ps) {${\bf G}_0$};
        \draw[-latex,line width=0.5mm, draw=gray] (0*\ps,0.08*\ps) -- (0*\ps,0.26*\ps);
        \node [scale=\scale, left] at (0*\ps,0.18*\ps) {$U_L$};
        \draw[latex-,line width=0.5mm, draw=gray] (1*\ps,0.08*\ps) -- (1*\ps,0.26*\ps);
        \node [scale=\scale, right] at (1*\ps,0.18*\ps) {$V_L$};

        \begin{scope}[shift={(0,3.4)}]
            \draw[gray] (0*\ps,0*\ps) circle (\r cm);
            \node [scale=\scale] at (0*\ps,0*\ps) {$\hat{q}_L$};
            \draw[draw=gray] (1*\ps,0*\ps) circle (\r cm);
            \node [scale=\scale] at (1*\ps,0*\ps) {$\hat{w}_L$};
            \draw[-latex,line width=0.5mm, draw=gray] (0.2 *\ps,0*\ps) -- (0.8*\ps,0*\ps);
            \node [scale=\scale, above] at (0.5*\ps,0*\ps) {${\bf G}_L$};
            \draw[-latex,line width=0.5mm, draw=gray] (0*\ps,0.08*\ps) -- (0*\ps,0.26*\ps);
            \node [scale=\scale, left] at (0*\ps,0.18*\ps) {$U_{L-1}$};
            \draw[latex-,line width=0.5mm, draw=gray] (1*\ps,0.08*\ps) -- (1*\ps,0.26*\ps);
            \node [scale=\scale, right] at (1*\ps,0.18*\ps) {$V_{L-1}$};
        \end{scope}
        \begin{scope}[shift={(0,6.6)}]
            \draw[-latex,line width=0.5mm, draw=gray] (0*\ps,0.08*\ps) -- (0*\ps,0.26*\ps);
            \node [scale=\scale, left] at (0*\ps,0.18*\ps) {$U_{1}$};
            \draw[latex-,line width=0.5mm, draw=gray] (1*\ps,0.08*\ps) -- (1*\ps,0.26*\ps);
            \node [scale=\scale, right] at (1*\ps,0.18*\ps) {$V_{1}$};
        \end{scope}
        \begin{scope}[shift={(0,1*\ps)}]
            \draw[gray] (0*\ps,0*\ps) circle (\r cm);
            \node [scale=\scale] at (0*\ps,0*\ps) {$\hat{q}_1$};
            \draw[draw=gray] (1*\ps,0*\ps) circle (\r cm);
            \node [scale=\scale] at (1*\ps,0*\ps) {$\hat{w}_1$};
            \draw[-latex,line width=0.5mm,draw=gray ] (0.2*\ps ,0*\ps) -- (0.8*\ps,0*\ps);
            \node [scale=\scale, above] at (0.5*\ps,0*\ps) {${\bf G}_1$};
        \end{scope}

        \node [scale=\scale] at (0.5*\ps,0.7*\ps) {\dots};
        \node [scale=\scale] at (0*\ps,0.7*\ps) {\vdots};
        \node [scale=\scale] at (1*\ps,0.7*\ps) {\vdots};
        \node [scale=\scale] at (5,-1.5) {~};
    }


==> FMM-Net (Version 200)/figs/rte_table.tex <==
 \begin{tabular}{||c c c c c||}
 \hline
 $N$ & h2nn &  MNN-$\mathcal{H}^2$-Mix &  MNN-$\mathcal{H}^2$-LC & conv\\
 \hline\hline
 320 &0.02350/0.02346 &   0.01197/0.01196&   0.00366/0.00383& 0.19538/0.19359\\
 640 &  0.02676/0.02687 &  0.06179/0.06381&   0.06271/0.06692&0.19683/0.19671\\
 1280 &   0.03240/0.03233 &  0.12397/0.125108&   0.16229/0.16438& 0.19686/0.19552\\ [1ex]
 \hline
\end{tabular}


==> FMM-Net (Version 200)/figs/rte_table_time.tex <==
 \begin{tabular}{||c c c c c||}
 \hline
 $N$ & h2nn &  MNN-$\mathcal{H}^2$-Mix &  MNN-$\mathcal{H}^2$-LC & conv\\
 \hline\hline
 320 &4.8127 &   2.7602&  0.7558& 1.1828\\
 640 &  8.6164 &  4.4834&   1.3990&2.0643\\
 1280 &   18.578 &  11.988&  2.7935&3.9055\\ [1ex]
 \hline
\end{tabular}


==> figs/ce_table_time.tex <==
 \begin{tabular}{||c c c c c||}
 \hline
 $N$ & h2nn &  MNN-$\mathcal{H}^2$-Mix &  MNN-$\mathcal{H}^2$-LC & conv\\
 \hline\hline
 320 &    3.9095 &   2.5115 &   0.7676 & 1.0347\\
 640 &    8.6155 &   4.4554 &   1.3959 & 2.2322\\
 1280 &   18.653 &   9.9784 &   2.5016 & 4.2035\\ [1ex]
 \hline
\end{tabular}



==> figs/f_l1.tex <==
\begin{figure}[H]
\centering
    \resizebox{0.4\textwidth}{!}{
    \tikz{
        \fill[white]  (0,0) rectangle (16,16);
        \foreach \i in {0,...,3}{
            \fill[blue!20!white]  (\i*4,\i*4) rectangle ++(4cm,4cm);
        }
        \foreach \i in {0,...,15}
        {
            \foreach \j in {0,...,4}
            {
                \pgfmathtruncatemacro{\r}{int(\closeDots[\i][\j])}
                \pgfmathtruncatemacro{\ii}{int(\closeDots[\i][0])}
                \draw [white,fill=white,opacity=1.0](\r,15-\ii) rectangle ++(1,1);
            }
        }
        \draw[step=1cm,gray!20!white] (0,0) grid (16,16);
        \draw[gray!80!white] (0,0) rectangle (16,16);
        \draw[step=4cm,gray,line width=0.34mm ] (0,0) grid (16,16);
        % \node [scale=3,left] at (-2,3.5) {Far block};
        % \draw[-latex,line width=1mm ] (-2,3.5) -- (0.5,3.5);
        % \node [scale=3,left] at (-2,11.5) {Interaction list};
        % \draw[-latex,line width=1mm ] (-2,11.5) -- (0.5,11.5);
        % \draw[white] (24,0) rectangle ++(1,1);
    }
    }
    \caption{Matrix $F_{L-1}$}
    \label{fig:inter_list}
\end{figure}


==> figs/rte_table_time.tex <==
 \begin{tabular}{||c c c c c||}
 \hline
 $N$ & h2nn &  MNN-$\mathcal{H}^2$-Mix &  MNN-$\mathcal{H}^2$-LC & conv\\
 \hline\hline
 320 &4.8127 &   2.7602&  0.7558& 1.1828\\
 640 &  8.6164 &  4.4834&   1.3990&2.0643\\
 1280 &   18.578 &  11.988&  2.7935&3.9055\\ [1ex]
 \hline
\end{tabular}

